Lost in Context Compaction: When LLM Systems Drop Side Constraints

When the context window is under pressure, LLM systems compact prior context to continue ongoing tasks. We study Side Constraints (SCs), user-issued instructions such as "do not delete any emails until I confirm," that constrain an LLM's behavior across subsequent turns but can be silently dropped during compaction. In an inbox experiment, an agent deleted emails without approval in 30/100 sessions after compaction, compared with none before compaction. To systematically evaluate SC preservation, we introduce CONPACT, an evaluation suite measuring semantic retention and downstream compliance across three scenarios: multi-turn chat, multi-turn tool use, and long-horizon research. The evaluated compactors retain only 17% of injected SCs on average. Loss occurs across compactors and settings, with retention varying by compactor, context length, SC framing, and injection location. We propose an SC extractor that maintains constraints separately from the task summary and appends them to the compacted context, achieving over 90% retention across all three scenarios without modifying the compactor or LLM. Code and data are available at https://github.com/ZhiqiEliWang/compaction-integrity.

==> tables/compliance_eval_group.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\caption{\textbf{Experiment groups for evaluating SC compliance under context compaction.} \textit{SC Injection} indicates the the order of injection relative to compaction (i.e., "Pre" means injecting SC before compaction). \textit{Compaction} is the main group of study that reflects the integrity issue of SC in real-world long context compaction.}
\label{tab:compliance-eval-groups}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Group} & \textbf{Context} & \textbf{SC Injection} & \textbf{Compaction} \\
\midrule
Long ctx w/ SC    & Full      & Yes & No  \\
Long ctx w/o SC & Full      & None & No  \\
\textbf{Compaction}  & Compacted & Pre  & Yes \\
Upper-bound          & Compacted & Post & Yes \\
\bottomrule
\end{tabular}
\end{table}

==> tables/rq1.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2pt}
\newcommand{\hd}[1]{{\fontsize{8}{9.5}\selectfont #1}}
\renewcommand{\arraystretch}{0.95}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l ccc ccc ccc @{}}
\toprule
& \multicolumn{3}{c}{\textbf{Hermes Agent}}
& \multicolumn{3}{c}{\textbf{OpenResearcher}}
& \multicolumn{3}{c}{\textbf{WildChat}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
& \hd{Retention} & \hd{Compaction} & \hd{Effective}
& \hd{Retention} & \hd{Compaction} & \hd{Effective}
& \hd{Retention} & \hd{Compaction} & \hd{Effective} \\
\textbf{Condition / Compactor}
& \hd{Rate} & \hd{Compliance} & \hd{Retention}
& \hd{Rate} & \hd{Compliance} & \hd{Retention}
& \hd{Rate} & \hd{Compliance} & \hd{Retention} \\
\midrule
Long ctx w/o SC          &   -- & 46.1 &   -- &   -- & 49.1 &   -- &   -- & 51.2 &   -- \\
Long ctx w/ SC           &   -- & 65.1 &   -- &   -- & 70.7 &   -- &   -- & 59.2 &   -- \\
\midrule
Recent-5                 &  0.4 & 48.4 &  4.6 &  0.0 & 52.0 &  6.3 &  0.0 & 53.3 &  5.1 \\
LLMLingua-2 T500         &  0.0 & 50.1 &  7.5 &  0.0 & 52.8 &  7.8 &  0.0 & 52.4 &  2.7 \\
Gemma-4-E4B (Anthropic)  & 12.5 & 55.0 & 16.8 &  3.6 & 54.5 & 11.5 &  2.0 & 55.7 & 10.5 \\
Qwen3-30B (Anthropic)    &  2.1 & 53.6 & 14.1 &  1.1 & 53.1 &  8.5 &  3.3 & 56.2 & 11.5 \\
gpt-oss-120b (Anthropic) & 18.5 & 58.5 & 23.8 &  8.4 & 53.9 & 10.6 &  1.3 & 54.6 &  8.1 \\
gpt-oss-120b (Pi)        & 36.3 & 60.7 & 27.8 & 19.6 & 56.2 & 15.2 &  0.0 & 51.2 &  0.0 \\
\arrayrulecolor{black!30}\midrule[0.3pt]\arrayrulecolor{black}
GPT-5.4-mini (Anthropic)$^\dagger$ & 53.7 & 72.3 & -- & 26.0 & 60.3 & -- & 28.3 & 64.9 & -- \\
GPT-5.4-mini (Pi)$^\dagger$        & 88.4 & 87.7 & -- & 98.0 & 85.7 & -- &  6.7 & 56.8 & -- \\
\bottomrule
\end{tabular*}
\caption{\textbf{SC retention and compliance across datasets and compactors ($N=750$; all values in \%).} The top two rows are uncompacted baselines; retention and effective retention do not apply to them. \textit{Retention Rate}: fraction of injected SCs preserved through compaction. \textit{Compaction Compliance}: compliance when probing on the compacted context (Eq.~\ref{eq:compliance}, $K_{\text{comp}}$), or on the full context for the baseline rows. \textit{Effective Retention}: compaction effect normalized by the upper-bound gain over the SC-free baseline (Eq.~\ref{eq:effective-retention}); upper-bound compliance is reported in Table~\ref{tab:rq1-upper-bound}. $^\dagger$GPT-5.4-mini is evaluated on a longer context (220K) to match its larger context window and on fewer trials ($N=300$) due to experiment cost, so the long-context baselines and effective retention are not available; details in Appendix~\ref{app:sec:gpt-5.4-mini}.}
\label{tab:rq1}
\end{table*}

